The Weak Supervision Landscape

Many ways of annotating a dataset for machine learning classification tasks that go beyond the usual class labels exist in practice. These are of interest as they can simplify or facilitate the collection of annotations, while not greatly affecting the resulting machine learning model. Many of these fall under the umbrella term of weak labels or annotations. However, it is not always clear how different alternatives are related. In this paper we propose a framework for categorising weak supervision settings with the aim of: (1) helping the dataset owner or annotator navigate through the available options within weak supervision when prescribing an annotation process, and (2) describing existing annotations for a dataset to machine learning practitioners so that we allow them to understand the implications for the learning process. To this end, we identify the key elements that characterise weak supervision and devise a series of dimensions that categorise most of the existing approaches. We show how common settings in the literature fit within the framework and discuss its possible uses in practice.

==> sections/dimensions.tex <==
\section{Dimensions of Weakly Supervised learning}

% In WSL we assume that the training data, $\tilde{\mathcal{D}}_{Train}$, is drawn from $\tilde{\mathcal{P}}$, which is a weak version of $\mathcal{P}$. On the other hand, the test data, $\mathcal{D}_{Test}$, is assumed to be drawn from the clean distribution, $\mathcal{P}$. The objective is to obtain a classifier $\tilde{h}$, trained on weak data, that performs well on $\mathcal{P}$. 

A first differentiator is whether each label provided corresponds to one instance, or whether it depends on a set of instances through an aggregation mechanism. When the noise is of the non-aggregate type then we assume we are provided with a noisy dataset~ $\tilde{\mathcal{D}}_n \sim P_{X,\tilde{Y}}^n$, instead of $\mathcal{D}_n \sim P_{X,Y}^n$, as would be expected in supervised learning. We assume the existence of the triplet $(X,~Y,~\tilde{Y})$, but we only get to observe $(X,~\tilde{Y})$. We will refer to $\mathbb{P}(\tilde{Y}~\mid~X,~Y)$ as the \textit{noise function}. We will then discuss WSL settings where the labels provided correspond to a group of instances, rather than being individually set. The label provided in these settings corresponds to a set of instances that we will refer to as a `bag'. Instead of being provided with a set of $\{(x_i,~y_i)\}_{i=1}^n$, we are provided with a set of $\{(x_i,~b_i)\}_{i=1}^n$ where $b_i$'s are bag indicators and  $\{(b_j,~t_j)\}_{j=1}^m$, where $t_j$'s are the corresponding provided labels. The labels in this case are of the form:
\begin{equation}
    t_j~=~g\big(\big\{y_i~\mid~i\in b_j\big\}\big)
\end{equation}
where we use $i\in b_j$ to imply that instance $i$ belongs to bag $j$, and $g$ is the label aggregation function. The distinction between the two is shown pictorially in Figure \ref{fig:agg_vs_nonagg}.

In what we discuss we are always interested in learning a classifier: $f:~\mathcal{X}~\to~\mathcal{Y}_{\textrm{Clean}}$ and in minimising ${\mathbb{P}_{X,Y}(f(X)\neq Y)}$\footnotemark.

\footnotetext{This corresponds to minimising the missclassification rate, but could be a different metric, that is with respect to the true data distribution $\mathbb{P}_{X,Y}$.}
% For example, in the settings of superset learning or partial label learning that we discuss below, for four classes, we could observe instances with two or three active labels, but would still be interested in predicting just one class.

\begin{figure}[!t]
    \centering
    \label{fig:agg_vs_nonagg}
    \includegraphics[width=0.85\linewidth]{figures/aggregated_vs_nonaggregate.drawio.pdf}
    \caption{Depiction of the difference between non-aggregate and aggregate noise functions. In the case of non-aggregate settings, there is a one-to-one relationship between instances and labels, while in the case of aggregate noise settings we observe one label per group. We note that a label could be one class, multiple or none, as we describe below.}
\end{figure}

% \begin{tcolorbox}
%     \begin{nfp}
%     \label{nfp:aggregate_ornot}
%     Are the labels provided a result of aggregation of multiple instances?
%     \end{nfp}
% \end{tcolorbox}



\subsection{Non-aggregated settings}

% Classification tasks can take different forms. It can be a binary classification task, where for example we might be interested in classifying an image as a dog or as a cat, or it can be a multi-class task, where we are classifying images of dogs according to their breed. In these cases we have a one-to-one relationship between an instance $\boldsymbol{x}_i$ and a label $\boldsymbol{y}_i$. There also exist classification tasks with structured data, such as classifying sequences at different granularity levels, or classifying pixels of images as background or foreground. We do not consider structured data in what follows. We now introduce necessary objects for the subsequent presentations.

% We will categorise non-aggregate weak supervision settings through two sets of dimensions. The first set of dimensions is concerned with properties of the noise process, while the second with the clean and weak label spaces.

% \begin{align*}
%     1:&\hspace{10pt}\mathbb{P}\big(\tilde{Y}~\mid~X=x,~Y=y\big)\\
%     2:&\hspace{10pt}y\in\mathcal{Y}_{Clean}~~and~~\tilde{y}\in\mathcal{Y}_{Weak}\\
% \end{align*}

The noise process is described as a \textit{Categorical} (\texttt{Cat}) distribution. This distribution is parametrised by a column of the \textit{mixing matrix}, $\boldsymbol{T}$, which is a non-negative column-wise stochastic matrix. The noise process is modelled as:

\begin{equation}
    \label{eq:noise_categorigal}
    \tilde{Y}~\mid~Y=\boldsymbol{y},~X=\boldsymbol{x}~\sim~\texttt{Cat}\big(\boldsymbol{T}\boldsymbol{y}\big)
\end{equation}
\todo[inline]{consider including an example of a mixing matrix here with some text}
With regards to properties of the noise function we will consider two: dependence on the instance and dependence on the true class. 

\subsubsection{true label space}
\subsubsection{agg vs nonagg}

\subsubsection{Dependence on instance}
We consider two cases: whether it is \textit{instance-dependent} or \textit{instance-independent}:
\begin{align*}
    &\textrm{Instance-independent noise (IIN)}:\\
    &\hspace{10pt} \mathbb{P}(\tilde{Y}=\tilde{y}~\mid~X=x,~Y=y)~=~\mathbb{P}(\tilde{Y}=\tilde{y}~\mid~Y=y),\\
    &\textrm{Instance-dependent noise (IDN)}:\\
    &\hspace{10pt} \mathbb{P}(\tilde{Y}=\tilde{y}~\mid~X=x,~Y=y)~\ne~\mathbb{P}(\tilde{Y}=\tilde{y}~\mid~Y=y).
    % \textrm{posterior-instance-dependent (PIDN)}:&\hspace{10pt} \mathbb{P}(\tilde{Y}=\tilde{y}~\mid~X=x,~Y=y) = \mathbb{P}(\tilde{Y}=\tilde{y}~\mid~\eta(x)=\eta,~Y=y)
\end{align*}

% \vspace{10pt}
% \begin{tcolorbox}
%     \begin{nfp}
%     \label{nfp:instance_dependence}
%     Dependence on instance: instance-independent noise (IIN) or instance-dependent noise (IDN).
%     \end{nfp}
% \end{tcolorbox}
% \vspace{10pt}
\subsubsection{Dependence on class}
With regards to the dependence on the true class we consider: \textit{symmetric} (/uniform) or \textit{asymmetric} (/class-conditional) with respect to the original classes. In the case of binary classification:

\begin{align*}
    &\textrm{Symmetric noise (SN)}:\\
    &\mathbb{P}(\tilde{Y}=0~\mid~X=x,~Y=1)=\mathbb{P}(\tilde{Y}=1~\mid~X=x,~Y=0),\\
    &\textrm{Asymmetric noise (ASN)}:\\
    &\mathbb{P}(\tilde{Y}=0~\mid~X=x,~Y=1)\neq\mathbb{P}(\tilde{Y}=1~\mid~X=x,~Y=0).
\end{align*}

In the case of multi-class classification, symmetric noise would imply:
\begin{align}
    \label{eq:multiclass_cnn}
    &\mathbb{P}(\tilde{Y}=e_u~\mid~X=x,~Y=e_i)\nonumber\\
    &\hspace{25pt}=~\mathbb{P}(\tilde{Y}=e_v~\mid~X=x,~Y=e_i)~=~\lambda,\\
    &\forall u,v,i \in [k],~u\neq v\neq i. \nonumber
\end{align}

We have asymmetric label noise when this does not hold. We summarise the second and third properties and their combinations in Table~\ref{table:noise_naming}.


\begin{table}[!t]
    \centering
        \begin{tabular}{|c|c|c|}\hline
                                      &\textbf{Asymmetric} &\textbf{Symmetric} \\\hline
        \textbf{Instance-dependent}   & ID-ASN                                             & ID-SN                                    \\
        \textbf{Instance-independent} & II-ASN (ASN)                                       & II-SN (SN)      \\\hline             
        \end{tabular}
    \caption{Table noting the naming conventions we use in the paper. In the case of binary classification symmetric and asymmetric are also known as uniform and class-conditional.}
    \label{table:noise_naming}
\end{table}

% In \cite{frenay2014comprehensive} the authors discuss the problem of label noise in general. Instead of presenting the axes of symmetric or asymmetric, and instance-dependent or instance-independent separately, they present them as one where: label noise completely at random (NCAR) occurs independently of
% the true class and of the values of the instance features, label noise that occurs at random (NAR) depends only on the true label. This can be used to model situations where some classes are more likely to be mislabelled than others, and lastly, label noise not at random (NNAR) is the more general case, where the mislabelling probability also depends on the feature values. The correspondence is as follows:
% \begin{align*}
%     \textrm{NCAR} &~~\to~~ \textrm{symmetric label noise (SN)}\\
%     \textrm{NAR} &~~\to~~ \textrm{asymmetric label noise (ASN)}\\
%     \textrm{NNAR} &~~\to~~ \textrm{instance-dependent noise (IDN) (SN or ASN)}\\
% \end{align*}

\subsubsection{Number of annotators}
\subsubsection{Availability of unlabelled data}
\subsubsection{Restriction on number of candidate classes}

% We will now discuss the second set of dimensions which is concerned with the label spaces. We assume that the clean label corresponds to one class, either in a binary or multi-class classification setting. We now look at several settings. 

% While this list is not exhaustive of the problems studied in the literature, it is a list of `base' problems ... \todo[inline]{elaborate}

% \begin{align*}
%     &\textrm{Multi-class (\& binary):}\\
%     &\hspace{10pt} \mathcal{Y}_k~=~ \big\{\boldsymbol{y}~\mid~\boldsymbol{y}\in\{0,~1\}^k,~\boldsymbol{1}^\top \boldsymbol{y}=1\big\}\\
%     &\textrm{Multi-class with unlabelled:}\\
%     &\hspace{10pt} \mathcal{Y}_{k+}~=~ \big\{\boldsymbol{y}~\mid~\boldsymbol{y}\in\{0,~1\}^k,~\boldsymbol{1}^\top \boldsymbol{y}\in\{0,1\}\big\}\\
%     &\textrm{Multi-label:}\\
%     &\hspace{10pt} \mathcal{Y}_{m, k} ~=~ \big\{\boldsymbol{y}~|~\boldsymbol{y}\in\{0,~1\}^k,~1\leq\boldsymbol{1}^{\top}\boldsymbol{y}\leq m\leq k\big\}\\
%     &\textrm{Multi-label restricted:}\\
%     &\hspace{10pt} \mathcal{Y}_{m, k}(z) ~=~ \big\{\boldsymbol{y}~|~\boldsymbol{y}\in\{0,~1\}^k,~1\leq\boldsymbol{1}^{\top}\boldsymbol{y}\leq m\leq k,~z\in \boldsymbol{y}\big\}\\
%     &\textrm{Multi-label multi-annotator with unlabelled:}\footnotemark\\
%     &\hspace{10pt} \mathcal{Y}_{m, k}^n ~=~ \big\{\boldsymbol{y}~|~\boldsymbol{y}\in\{0,~1\}^{k\times n},~0\leq\boldsymbol{y}^{\top}\boldsymbol{1}\leq m\leq k\big\}\\
% \end{align*}

% \footnotetext{The inequalities are to be understood as elementwise.}


% MPN: table backup, I am working with a copy below
%\begin{table*}[t!]
%\centering
%\begin{tabular}{|c||c|c|c|}\hline
%Name           & True labels & Weak labels & Mixing matrix\\\hline\hline
%Noisy Labels & $\mathcal{Y}_k$                                & $\mathcal{Y}_k$                                 & $\boldsymbol{T}\in\mathbb{R}^{k\times k}$          \\\hline
%Partial Labels & $\mathcal{Y}_k$                                & $\mathcal{Y}_{m, k}$                   & $\boldsymbol{T}\in\mathbb{R}^{(2^k-2)\times k}$ \\\hline
%Superset Learning       & $\mathcal{Y}_k$                                & $\mathcal{Y}_{m, k}(z)$                & $\boldsymbol{T}\in\mathbb{R}^{(2^k-2)\times k} $ \\\hline
%Complementary Labels       & $\mathcal{Y}_k$                                & $\mathcal{Y}_{m, k}(z)$                & $\boldsymbol{T}\in\mathbb{R}^{(2^k-2)\times k}$\\\hline
%% Multi-label to Multi-label      & $\mathcal{Y}_{{}_{\leq}m, k}$                               & $\mathcal{Y}_{{}_{\leq}m, k}(z)$                & $\boldsymbol{T}\in\mathbb{R}^{(2^m-1)\times (2^m-1)}$\\\hline
%Semi-supervised Learning & $\mathcal{Y}_k$                                & $\mathcal{Y}_{k+1}$                                 & $\boldsymbol{T}\in\mathbb{R}^{k+1\times k}$ \\\hline
%Positive-Unlabelled & $\mathcal{Y}_2$                                & $\mathcal{Y}_3$                                 & $\boldsymbol{T}\in\mathbb{R}^{3\times 2}$           \\\hline
%Multi-Positive and Unlabeled & $\mathcal{Y}_k$                                & $\mathcal{Y}_{k+1}$                                 & $\boldsymbol{T}\in\mathbb{R}^{(k+1)\times k}$           \\\hline
%Multiple annotators (n) & $\mathcal{Y}_k$                                & $\mathcal{Y}_k^n$                                 & $\boldsymbol{T}\in\mathbb{R}^{k\times k}$          &\hline
%\end{tabular}
%\caption{Describing various WSL settings according to the label-space of true labels and noisy labels, and the mixing matrix used to model the noise process.}
%\label{table:noise_settings}
%\end{table*}

\begin{table*}[t!]
\caption{Describing various WSL settings according to the label-space of true labels and noisy labels, and the mixing matrix used to model the noise process.}
\label{table:noise_settings}
\centering
\begin{tabular}{|c||c|c|c|}\hline
Name & True labels & Weak labels & Mixing matrix\\\hline\hline
Noisy Labels & $\mathcal{Y}_k$ & $\mathcal{Y}_k$ & $\boldsymbol{T}\in\mathbb{R}^{k\times k}$ \\\hline
Partial Labels & $\mathcal{Y}_k$ & $\mathcal{Y}_{m, k}$ & $\boldsymbol{T}\in\mathbb{R}^{(2^k-2)\times k}$ \\\hline
Superset Learning & $\mathcal{Y}_k$ & $\mathcal{Y}_{m, k}(z)$ & $\boldsymbol{T}\in\mathbb{R}^{(2^k-2)\times k} $ \\\hline
Complementary Labels & $\mathcal{Y}_k$ & $\mathcal{Y}_{m, k}(z)$ & $\boldsymbol{T}\in\mathbb{R}^{(2^k-2)\times k}$\\\hline
% Multi-label to Multi-label & $\mathcal{Y}_{{}_{\leq}m, k}$ & $\mathcal{Y}_{{}_{\leq}m, k}(z)$ & $\boldsymbol{T}\in\mathbb{R}^{(2^m-1)\times (2^m-1)}$\\\hline
Semi-supervised Learning & $\mathcal{Y}_k$ & $\mathcal{Y}_{k+1}$ & $\boldsymbol{T}\in\mathbb{R}^{(k+1)\times k}$ \\\hline
Positive-Unlabelled & $\mathcal{Y}_2$ & $\mathcal{Y}_3$ & $\boldsymbol{T}\in\mathbb{R}^{3\times 2}$ \\\hline
Multi-Positive and Unlabeled & $\mathcal{Y}_k$ & $\mathcal{Y}_{k+1}$ & $\boldsymbol{T}\in\mathbb{R}^{(k+1)\times k}$ \\\hline
Multiple annotators (n) & $\mathcal{Y}_k$ & $\mathcal{Y}_k^n$ & $\boldsymbol{T}\in\mathbb{R}^{k\times k}$ \\\hline
\end{tabular}
\end{table*}


\paragraph{Noisy labels (Flipping noise)} In this setting instances switch labels with a certain probability. This type of noise could be introduced when the data is labelled by an annotator who is not an expert. This nicely extends to the setting where there are multiple such annotators. Some of the first works date back to the works of \cite{angluin1988learning} where the focus was on understanding the impact of symmetric label noise on learnability. In this setting the clean and noisy label spaces are the same.
\begin{align*}
    \mathcal{Y}_k&~\to~\mathcal{Y}_k\\
    \boldsymbol{T}&~\in~\mathbb{R}^{k\times k}
\end{align*}

where:
\begin{equation}
    \label{eq:multiclass_label_space}
    \mathcal{Y}_k~=~ \big\{\boldsymbol{y}~\mid~\boldsymbol{y}\in\{0,~1\}^k,~\boldsymbol{1}^\top \boldsymbol{y}=1\big\}
\end{equation}
An example of a mixing matrix for flipping noise in the case of binary classification:
\begin{equation*}
    \centering
    \bordermatrix{& \textcolor{blue}{\textrm{+ve}} & \textcolor{blue}{\textrm{-ve}}\cr
      \textcolor{blue}{\textrm{+ve}} & 1-\gamma_0 & \gamma_1 \cr
      \textcolor{blue}{\textrm{-ve}} & \gamma_0 & 1-\gamma_1}
\end{equation*}
where in the case of $\gamma_0=\gamma_1$ we would have symmetric label noise, while for $\gamma_0\neq\gamma_1$ it would be asymmetric label noise. In the case of instance-independent noise, $\gamma_0$ and $\gamma_1$ are constants, i.e. all instances have their label flipped with same probability. On the other hand, in the case of instance-dependent noise, $\gamma_0$ and $\gamma_1$ could be functions of $x$, where $\gamma_0(x_i)\neq\gamma_1(x_j)$.


\paragraph{Superset Learning \& Complementary Labels} In this setting an observed label could be any combination of class labels, subject to the constraint that this combination contains the true label. For example in the case of multi-class classification with three classes, for a true label $[001]$ we could observe $[011]$ or $[101]$, but not $[110]$. Superset learning has been studied in the literature under different names such as `learning with partial-labels' (see below) and `learning with ambiguous labels'. Motivating use-cases for superset learning setting include picture tags and bird singing \cite{liu2012conditional}. Some of the earlier works on the topic include \cite{grandvalet2002logistic} and \cite{jin2002learning} where the setting is referred to as `partial-labels' and `multiple labels' respectively. An example of a transition matrix for superset learning:
% Another early work is that of \cite{ambroise2001learning}.
\begin{equation*}
    \bordermatrix{
    & \textcolor{blue}{\textrm{001}} & \textcolor{blue}{\textrm{010}} & \textcolor{blue}{\textrm{100}}\cr
  \textcolor{blue}{\textrm{001}} & \alpha_0 & 0 & 0\cr                % 001
  \textcolor{blue}{\textrm{010}} & 0 & \beta_0 & 0\cr               % 010
  \textcolor{blue}{\textrm{100}} & 0 & 0 & \gamma_0\cr                % 100
  \textcolor{blue}{\textrm{110}} & 0 & \beta_1 & \gamma_1\cr         % 011
  \textcolor{blue}{\textrm{101}} & \alpha_1 & 0 & 1-\gamma_0-\gamma_1\cr        % 101
  \textcolor{blue}{\textrm{011}} & 1-\alpha_0-\alpha_1 & 1-\beta_0-\beta_1 & 0\cr         % 110
%   \textcolor{blue}{\textrm{111}} & 1 - \sum_i \alpha_i & 1 - \sum_i \beta_i  & 1 - \sum_i \gamma_i\cr    % 111
 }
\end{equation*}
\vspace{5pt}

We note that in the case of superset learning ${\mathbb{P}(\tilde{Y}=\tilde{y}~\mid~Y=y,~y\notin \tilde{y})=0}$, where we abuse notation and use $\tilde{y}$ both as a label and as a set. In words: in superset learning it is always the case that the observed noisy label/set includes the true label. On the other hand it doesn't disallow zero-probability when $z$ does indeed cover $y$, i.e. $\mathbb{P}(\tilde{Y}=\tilde{y}~\mid~Y=y,~y\in \tilde{y})\geq0$. In the case of learning from partial labels, there are no such restrictions. Learning from complementary labels refers to the setting where one is provided with a set of instances, \textit{none} of which is the true label \cite{ishida2017learning}. By flipping this information around we are back at superset learning.

\begin{align*}
    \mathcal{Y}_k&~\to~\mathcal{Y}_{m,k}(z)\\
    \boldsymbol{T}&~\in~\mathbb{R}^{(2^k-2)\times k}
\end{align*}

where:
\begin{equation}
    \label{eq:superset_label_space}
    \mathcal{Y}_{m, k}(z)= \big\{\boldsymbol{y}~|~\boldsymbol{y}\in\{0,~1\}^k,~1\leq\boldsymbol{1}^{\top}\boldsymbol{y}\leq m\leq k,~z\in \boldsymbol{y}\big\}
\end{equation}

We define it as an extension of the multi-label set (Eq. \ref{eq:partial_label_space}) that accepts an input. We abuse notation and use $\boldsymbol{y}$ both as a vector and as a set and with $z\in\boldsymbol{y}$ we imply that $\boldsymbol{y}$ covers $z$, i.e. has a non-zero entry wherever $z$ has a non-zero entry.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/sset_pl.drawio.pdf}
%     \caption{Depiction of the difference between superset learning and partial labels. For both, per instance, we could observe more than one label. In the case of superset learning though one of them is necessarily correct (green), while in the case of partial labels all of them could be wrong (red).}
%     \label{fig:sset_vs_pl}
% \end{figure}

\paragraph{Partial Labels} In the literature PLL is often used to refer to what we refer to as superset learning setting. The setting of PLL is similar to that of superset learning but where there is no restriction that the observed weak label includes the true label.


\begin{align*}
    \mathcal{Y}_k&~\to~\mathcal{Y}_{m,k}\\
    \boldsymbol{T}&~\in~\mathbb{R}^{(2^k-2)\times k}
\end{align*}


where:
\begin{equation}
    \label{eq:partial_label_space}
    \mathcal{Y}_{m, k} ~=~ \big\{\boldsymbol{y}~|~\boldsymbol{y}\in\{0,~1\}^k,~1\leq\boldsymbol{1}^{\top}\boldsymbol{y}\leq m\leq k\big\}
\end{equation}

\begin{equation}
    \label{eq:partial_label_space}
    \mathcal{Y}^n_{m, k} ~=~ \big\{\boldsymbol{y}~|~\boldsymbol{y}\in\{0,~1\}^{k\times n},~l\leq\boldsymbol{1}^{\top}\boldsymbol{y}\leq m\leq k\big\}
\end{equation}

% The distinction between superset learning and learning with partial labels is shown pictorially in Fig~\ref{fig:sset_vs_pl}. 
In both settings the set of potential observations extends from $k$ to $2^k-2$. While standard presentations of the settings consider $2^k-1$, we choose to exclude the all inclusive potential observation and instead consider it as an extra dimension.


\paragraph{Semi-supervised Learning} Semi-supervised learning (SSL) \cite{chapelle2009semi} is another very well studied setting. In this case, on top of the usual supervised dataset, we are also provided with an unlabelled dataset. 

\begin{align*}
    \mathcal{Y}_k&~\to~\mathcal{Y}_{k+}\\
    \boldsymbol{T}&~\in~\mathbb{R}^{(k+1)\times k}
\end{align*}

where:
\begin{equation}
    \label{eq:ssl_labelspace}
    \mathcal{Y}_{k+}~=~ \big\{\boldsymbol{y}~\mid~\boldsymbol{y}\in\{0,~1\}^k,~\boldsymbol{1}^\top \boldsymbol{y}\in\{0,1\}\big\}
\end{equation}
and is an extension of the multi-class label space (Eq. \ref{eq:multiclass_label_space}) that allows for no classes to be provided. An example of a transition matrix for semi-supervised learning:

\begin{equation*}
     \bordermatrix{& \textcolor{blue}{\textrm{+ve}} & \textcolor{blue}{\textrm{-ve}}\cr
      \textcolor{blue}{\textrm{+ve}} & 1-\gamma_0 & 0 \cr
      \textcolor{blue}{\textrm{na}} & \gamma_0 & \gamma_1 \cr
      \textcolor{blue}{\textrm{-ve}} & 0 & 1-\gamma_1}\\
\end{equation*}

\paragraph{Positive-Unlabelled (PU) Learning}
Learning with positive and unlabelled instances, or PU learning, is the setting of binary classification where the training dataset only consists of positive and unlabelled instances. Situations where PU learning arises include: medical records where only known previous diseases are listed and personalised advertising where visited pages and clicks are the positive cases \cite{bekker2020learning}. 

\begin{align*}
    \mathcal{Y}_2&~\to~\mathcal{Y}_{2+}\\
    \boldsymbol{T}&~\in~\mathbb{R}^{3\times 2}
\end{align*}

An example of a mixing matrix for PU learning: 
\begin{equation*}
    \bordermatrix{& \textcolor{blue}{\textrm{+ve}} & \textcolor{blue}{\textrm{-ve}}\cr
      \textcolor{blue}{\textrm{+ve}} & 1-\gamma_0 & 0 \cr
      \textcolor{blue}{\textrm{-ve}} & 0 & 0 \cr
      \textcolor{blue}{\textrm{na}} & \gamma_0 & 1}
\end{equation*}

The setting of PU learning has also been extended to the multi-class case, under the name 
Multi-Positive and Unlabeled learning, where labeled data from multiple positive classes are provided for training along with unlabeled data from a mixture of the positive classes and a negative class \cite{xu2017multi}.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/wsl_dimensions.drawio.pdf}
%     \caption{A pictorial illustration of the set of dimensions that describe the relationship between the clean and weak label spaces, for the case of non-aggregate noise functions.}
%     \label{fig:nonaggregate_wsl_cube}
% \end{figure}

\paragraph{Multiple annotators (Noisy labels)} Assuming we have $m$ annotators, we also have potentially $m$ distinct mixing matrices. Therefore, $\tilde{Y}^n~=~\big\{\tilde{Y} \sim \texttt{Cat}\big(\boldsymbol{T}_j\boldsymbol{y}\big)\big\}_{j=1}^n$, where $\boldsymbol{T}_j$ denotes the $j^{th}$ annotator's mixing matrix. 

% With $\mathcal{Y}_k^n$ we imply the cartesian product of $\mathcal{Y}_k$ $n$ times, i.e. $\mathcal{Y}_k^n = \mathcal{Y}_k \times \mathcal{Y}_k \times \dots \times \mathcal{Y}_k$.

\begin{align*}
    \mathcal{Y}_k&~\to~\mathcal{Y}^{n}_{k}\\
    \Big\{\boldsymbol{T}&~\in~\mathbb{R}^{k\times k}\Big\}_{j=1}^n
\end{align*}

where:
\begin{equation}
    \label{eq:multiannotator_labelspace}
    \mathcal{Y}_{m, k}^n ~=~ \big\{\boldsymbol{y}~|~\boldsymbol{y}\in\{0,~1\}^{k\times n},~0\leq\boldsymbol{y}^{\top}\boldsymbol{1}\leq m\leq k\big\}
\end{equation}

and where the inequalities should be understood as elementwise.

% In Table \ref{table:noise_settings} we summarise WSL settings with regards to the label space structures for the true and weak label spaces, and by describing the noise process. We have presented several non-aggregate weak supervision settings from which we extract the following dimensions, on how they affect the weak label space:
% \begin{itemize}
%     \item Number of annotators,
%     \item Availability of unlabelled data,
%     \item Restriction on number of candidate classes per instance (per annotator).
% \end{itemize}

% and these affect the noise function:
% \begin{itemize}
%     \item Dependence on the instance,
%     \item Dependence on the true class.
% \end{itemize}

In Figure \ref{fig:weak_label_example} we have an example of a possible weak label, with the aim of showing the impact of the different dimensions on its structure.

% We note that the settings could of course be combined. Examples include `semi-supervised learning', where on top of the existing weak supervision setting the provided data also includes unlabelled instances. Similarly, for the case of `multiple annotators' it could be the case that annotators are not only subject to flipping noise -as illustrated above- but rather are subject to more complex ones, and maybe each with different one. Noise could also depend on exogenous variables such as the case of having multiple datasets, each with different label quality.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/example_weak_label.drawio.pdf}
    \caption{An example of a non-aggregate weak label. For this case we consider six base classes and access to four annotators. This example showcases the three dimensions shown in Figure \ref{fig:nonaggregate_wsl_cube}. (1) Transitioning from one to multiple annotators, (2) Annotators can provide an empty annotation set (see annotator 3), and (3) Annotators can provide an annotation set with more than one candidate classes (see annotators 1 and 2).}
    \label{fig:weak_label_example}
\end{figure}

% \todo[inline]{this might need refinement; consider swapping u,v and i, for u, and i,j}
% For noise function property 3 we stated conditions that hold for flipping noise. In the more general case we can restate Eq.~\ref{eq:multiclass_cnn} as follows:
% \begin{align}
%     \label{eq:multiclass_cnn}
%     &\mathbb{P}(\tilde{Z}=z_u~\mid~X=x,~Y=e_i)~=~\mathbb{P}(\tilde{Z}=z_v~\mid~X=x,~Y=e_i)~=~\lambda,\\
%     &\hspace{5pt}\forall u,v,i \in [k],~u\neq v\neq i. \nonumber
% \end{align}
% This should also be subject to the condition that $e_i\in z_u$ for the case of superset learning.

% \todo[inline]{this needs refinement}
% What we now discuss departs from what we have presented so far as the output of the noise function is not individual.

\subsection{Aggregated noise settings}
% \todo[inline]{need to say something on how for all previous settings the we described a probabilistic data generating process, while now we don't}

We will now discuss WSL settings where the labels provided correspond to a group of instances, rather than corresponding to one individual instance only. As already discussed, we are provided with a set of $\{(x_i,~z_i)\}_{i=1}^n$ where $z_i$'s are bag indicators and  $\{(b_j,~t_j)\}_{j=1}^m$, where $b_j$'s are bag indicators and $t_j$'s are the corresponding provided labels. The labels in this case are of the form:
\begin{equation}
    t_j~=~g\Big(\big\{y_i~\mid~i\in b_j\big\}\Big)
\end{equation}
where we use $i\in b_j$ to imply that instance $i$ belongs to bag $j$, and $g$ is the label aggregation function. We will now see a few different forms of $g$.


\paragraph{Multiple Instance Learning} Multiple instance learning (MIL) is usually considered in the binary classification case. The label provided for each bag is an indicator of the presence of the positive class. It was first introduced in \cite{dietterich1997solving} with the motivation of drug activity prediction.

\begin{equation*}
    g(y_1, \dots, y_n)~=~max\big(y_{[1..n]}\big)
\end{equation*}

In the case of the multi-class classification settings we would have the following:
\begin{equation*}
    g(y_1, \dots, y_n;~c)~=~max\big(y_{[1..n]};~c\big)~=~max\big(\big\{y_{i,c}\big\}_{i=1}^n\big)
\end{equation*}

In words: is there at least one element of class $c$ in the input set?

\paragraph{Learning from Label Proportions}
In the case of learning with label proportions (LLP) the aggregation function is the count function for each of the classes. LLP was introduced in \cite{musicant2007supervised} with the motivation of learning with mass spectrometry data.

\begin{equation*}
    g(y_1, \dots, y_m)~=~\Bigg[\sum_{i=1}^{m} y_{i,0},~\cdots,~\sum_{i=1}^{m} y_{i,c}\Bigg]
\end{equation*}

In LLP for each bag we are provided with the proportions of each of the classes. PU Learning was presented as being a non-aggregate noise setting, but under certain conditions it can also be seen as a case of aggregate noise, and more specifically learning from label proportions. In PU Learning we are provided with a set of positive data and a set of unlabelled data. In the case of knowing the portions of positives and negatives in the unlabelled set, we can view PU Learning as an instance of learning with label proportions with two bags (where one of them is pure).

\paragraph{Generalised Multiple-Instance Learning}
In \cite{scott2005generalized} the authors extend MIL, from requiring at least one positive instance in a bag, to requiring $r$.
\begin{equation*}
    g(y_1, \dots, y_m)~=~\boldsymbol{1}\Big\{\sum_{i=1}^{m} y_{i} \geq r\Big\}
\end{equation*}

\subsubsection{Discussion}
Similarly to the non-aggregate case, aggregate settings could be extended to the case of having access to unsupervised data or multiple annotators. Instance-dependence has a different meaning in this case though. While previously it had to do with whether the noise function was uniform across all instances, in this case it has to do with bag creation and intra-bag similarities \cite{zhou2009multi,carbonneau2018multiple,scott2020learning}

\subsection{Summary}
In the previous sections we discussed several dimensions that can be used to categorise weak supervision settings, that we summarise in Figure \ref{fig:wsl_table}. In this table we note the six dimensions we have identified, with the distinction between aggregate and non-aggregate as the most important.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/wsl_table_2.drawio.pdf}
    \caption{Caption}
    \label{fig:wsl_table}
\end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{chapters/weaksupervision/figures/wsl_axes.drawio (1).pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% \begin{tcolorbox}
%     \textbf{Primary NFP 1.:}~Are the labels provided a result of aggregation of multiple instances?\\
%     \textbf{Primary NFP 2.:}~Dependence on instance: instance-independent noise (IIN) vs. instance-dependent noise (IDN).\\
%     \textbf{Primary NFP 3.:}~Dependence on class: asymmetric noise (ASN) vs. symmetric noise (SN).\\
%     \textbf{Primary NFP 4.:}~How are the true label and noisy label spaces related?
% \end{tcolorbox}

% \begin{tcolorbox}[colback=pink]
%     \textbf{Secondary NFP 1.:}~Is there just one annotator, or several? Do we have access to multiple datasets, each with different label quality?\\
%     \textbf{Secondary NFP 2.:}~Besides the weak data, is there also unsupervised data?
% \end{tcolorbox}


\subsection{Open research problems}
% \begin{adjustwidth}{0.50cm}{}
% \paragraph{Multiple annotators for Partial Labels and Superset learning}
% While the setting of multiple annotators is well studied in the literature it is focused on the case where each annotator provides an annotation consisting of one potentially noisy label. The setting where annotators are permitted to provide a set of labels -either under the superset learning assumption or not- could allow for more flexibility in the data collection phase.
% \end{adjustwidth}

\paragraph{Symmetric and Asymmetric noise for Partial Labels and Superset learning}
In the case of binary and multi-class classification with noisy labels, the distinction between symmetric and asymmetric label noise is important as in the former -under mild assumptions- the Bayes classifier mirrors the behaviour of the Bayes classifier under a clean distribution. How does this distinction translate when we are dealing with superset learning or learning from partial labels?

\paragraph{Symmetric and Asymmetric noise for aggregate noise functions}
Similarly to the discussion above; the distinction between symmetric and asymmetric label noise is not studied in the case of aggregate noise functions.



==> sections/open_problems.tex <==

\section{Open research problems}
\label{section:open_problems}
% \begin{adjustwidth}{0.50cm}{}
% \paragraph{Multiple annotators for Partial Labels and Superset learning}
% While the setting of multiple annotators is well studied in the literature it is focused on the case where each annotator provides an annotation consisting of one potentially noisy label. The setting where annotators are permitted to provide a set of labels -either under the superset learning assumption or not- could allow for more flexibility in the data collection phase.
% \end{adjustwidth}

\paragraph{Symmetric and Asymmetric noise for Partial Labels and Superset learning}
In the case of binary and multi-class classification with noisy labels, the distinction between symmetric and asymmetric label noise is important as in the former -under mild assumptions- the Bayes classifier mirrors the behaviour of the Bayes classifier under a clean distribution. How does this distinction translate when we are dealing with superset learning or learning from partial labels?

\paragraph{Unified view of aggregate WSL settings}
In the case of non-aggregate settings we have seen how several seemingly disparate settings can be viewed as special cases of Equation \ref{eq:noise_categorigal}. This is not only a matter of aesthetics, but more importantly allows for the transferability of methods and theory. In the case of aggregate WSL settings, while we have Equation \ref{eq:aggregate_function} showing how aggregation is abstracted away, it doesn't strengthen the understanding of theory, or allow for algorithms to be applied across settings. 



==> sections/todos.tex <==





\todo[inline]{algorithm: how to learn mixing matrix?}
\todo[inline]{cost of annotation?}

